Cross attentive pooling for speaker verification

The goal of this paper is text-independent speaker verification where utterances come from 'in the wild' videos and may contain irrelevant signal. While speaker verification is naturally a pair-wise problem, existing methods to produce the speaker embeddings are instance-wise. In this paper, we propose Cross Attentive Pooling (CAP) that utilizes the context information across the reference-query pair to generate utterance-level embeddings that contain the most discriminative information for the pair-wise matching problem. Experiments are performed on the VoxCeleb dataset in which our method outperforms comparable pooling strategies.

==> unused.tex <==
% % $\dag$ Note that \cite{kye2020meta} uses the same ResNet-34 network but with twice as many filters in all layers.
% \begin{table*}[t]
% \renewcommand\arraystretch{1.1}
% \centering
%     \caption{Comparison with various aggregation methods. {\bf NP}: Normalised Prototypical, {\bf AP}: Angular Prototypical, {\bf TAP}: Temporal Average Pooling, {\bf SAP}: Self-Attentive Pooling, {\bf CAP}: Cross-Attentive Pooling.} 
%     \vspace{+0.1in}
% % \resizebox{1\textwidth}{!}{
% % 	\small
%  \begin{tabular}{c c c c c | c c }
% \toprule 
% & Feature extractor & Feature & Objective & Aggregation & MinDCF
%  & EER (\%) \\ \midrule
% Xie \textit{et al.}~\cite{Xie19a}& Thin ResNet-34 & Spectrogram-257 & Softmax & GhostVLAD &  - & 3.22 \\ 
% Jung \textit{et al.}~\cite{SPE} & ResNet-34 & MFB-64 & A-Softmax & SPE &  - & 2.61 \\
% Yu \textit{et al.}~\cite{yu2019ensemble} & ResNet-50 & Spectrogram-512 & EAM-Softmax & TAP & - & 2.94 \\
% Chung \textit{et al.}~\cite{chung2020defence}& Fast ResNet-34 & MFB-40 & AP & TAP &  0.176 & 2.22 \\ 
% Kye \textit{et al.}~\cite{kye2020meta} & ResNet-34 & MFB-40 & NP + Softmax & TAP &  - & 2.08 \\ \midrule

% % Ours & Fast ResNet-34 & MFB-40 & NP & TAP &  0.192 & 2.33 \\
% % Ours & Fast ResNet-34 & MFB-40 & NP & SAP &  0.194 & 2.49 \\ 
% % Ours & Fast ResNet-34 & MFB-40 & NP & CAP &  - & - \\ \midrule

% \textbf{Ours} & Fast ResNet-34 & MFB-40 & NP + Softmax & TAP &  0.154 $\pm$ 1e-4 & 2.08 $\pm$ 0.01 \\
% \textbf{Ours} & Fast ResNet-34 & MFB-40 & NP + Softmax & SAP &  0.156 $\pm$ 3e-4 & 2.09 $\pm$ 0.01\\ 
% \textbf{Ours} & Fast ResNet-34 & MFB-40 & NP + Softmax & CAP & \textbf{0.148 $\pm$ 0.01} & \textbf{1.89 $\pm$ 0.06}   \\ \bottomrule 

%  \end{tabular}
% % }
%  \vspace{-0.15in}
%     \label{tbl:comparison}
% \end{table*}

==> unused2.tex <==
% \begin{table}[t]
% \renewcommand\arraystretch{1.1}
% \centering
%     \caption{Comparison with various aggregation methods. $\dag$ Note that \cite{kye2020meta} uses the same ResNet-34 network but with twice as many filters in all layers. {\bf NP}: Normalised Prototypical, {\bf AP}: Angular Prototypical, {\bf TAP}: Temporal Average Pooling, {\bf SAP}: Self-Attentive Pooling, {\bf CAP}: Cross-Attentive Pooling.} 
%     \vspace{+0.1in}
%  \begin{tabular}{c c | r r }
% \toprule 
% Objective & Aggregation & MinDCF
%  & EER (\%) \\
%  \midrule
% AP~\cite{chung2020defence} & TAP &  - & 2.22 \\ 
% NP + Softmax~\cite{kye2020meta}$\dag$ & TAP &  - & 2.08 \\ \midrule

% NP & TAP &  0.192 & 2.33 \\
% NP & SAP &  0.194 & 2.49 \\ 
% NP & CAP &  - & - \\ \midrule

% NP + Softmax & TAP &  0.164 & 2.13 \\
% NP + Softmax & SAP &  0.161 & 2.08 \\ 
% NP + Softmax & CAP & \textbf{0.148 $\pm$ 0.01} & \textbf{1.88 $\pm$ 0.06}   \\ \bottomrule 

%  \end{tabular}

%  \vspace{-0.15in}
%     \label{tbl:comparison}
% \end{table}
